Higgs-Yukawa model in chirally-invariant lattice field theory

Non-perturbative numerical lattice studies of the Higgs-Yukawa sector of the standard model with exact chiral symmetry are reviewed. In particular, we discuss bounds on the Higgs boson mass at the standard model top quark mass, and in the presence of heavy fermions. We present a comprehensive study of the phase structure of the theory at weak and very strong values of the Yukawa coupling as well as at non-zero temperature.

==> figures/StrongYukawaCoupling/LargeYukawaCoupling.tex <==
%
%
So far, it is not clear if the Higgs-Yukawa model at large unrenormalized Yukawa couplings differs from the model in a region of weak couplings. A first step in a detailed analysis and hence a deeper understanding of the model in this region is the investigation of the bulk phase transition. It can be shown, that the Higgs-Yukawa model reduces to a pure scalar non-linear $\sigma$-model at infinite Yukawa couplings~\cite{Abada:1990ds}, and hence becomes trivial at a certain cutoff. However, it is not clear what happens at large but finite Yukawa couplings. To be able to detect any differences to a Gaussian (trivial) theory the critical exponents of the phase transition are investigated and compared to the ones of the O(4) model. If it turns out that this region is indeed different it would be very interesting to investigate the possibility of heavy fermions which give rise of a fourth generation here.

The magnetization, Eq.~(\ref{eq:mag}), can act as an order parameter to identify and determine the order of the phase transition. In FIG. \ref{MagAtLargeY}, the magnetization for the Higgs-Yukawa model are shown for two $\kappa$ values and the O(4) model in dependence of the volume. The two phases can be clearly distinguished and the phase transition is washed out because of finite volume effects as mentioned previously. In addition, the magnetization never is zero due to finite volume effects.

The absence of any discontinuities in the magnetization is a strong evidence for a second order phase transition in all three depicted cases. In general, second order phase transitions are classified through their critical exponents and the question arises if these exponents are different from the standard model predicted ones in the region of large Yukawa couplings. Hence, a careful investigation of susceptibility and  Binder's cumulant will be presented in the following. 

%%%%%%%%%%%%%%%%%%%%%%
%Picture%%%%% Magnetization at large Y 
\begin{figure}[H]
	\begin{center}
	$	
	\begin{array}{ccc}
		\hspace*{-0.5cm}  \input{./pictures/StrongYukawaCoupling/mag_kap006.tex} &
		\hspace*{-1.2cm}  \input{./pictures/StrongYukawaCoupling/mag_kap000.tex} &
		\hspace*{-1.2cm}  \input{./pictures/StrongYukawaCoupling/mag_O4.tex} 
	\end{array}
	$	
	\end{center}
\vspace*{-0.5cm}
\caption[Magnetization at large Yukawa couplings.]{Magnetization $\left< m\right>$ for the Higgs-Yukawa model at $\kappa=0.06$ (left), $\kappa=0.00$ (middle) and the O(4) model (right) for various volumes. The x axis on the O(4) model plot is inverted to match optically with the Higgs-Yukawa model. The absence of discontinuities in $\left< m\right>$ is a strong evidence for a second order phase transition.}	
\label{MagAtLargeY}
\end{figure} %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
The critical exponents can be calculated by using the finite size scaling of the susceptibility, Eq.~(\ref{eq:susc_def}). It is shown in FIG.~\ref{SusAtLargeY}. This quantity diverges at the critical points in the infinite volume limit. Finite-size effects result in the crossover from this bulk behavior to the finite-volume scaling behavior in lattice calculations. As mentioned before in Eq.~(\ref{eq:susc_scaling}), the finite size scaling is predicted by the RGE, with the modification resulting from scaling violation,
\begin{equation}
	\chi_{m}\left(t, L\right)\cdot L_s^{-\gamma/\nu} =  g\left(t L_s^{1/\nu}\right)\text{,\, with \,} t=\left[T/\left(T_c^{(L=\infty)} - C\cdot L_s^{-b}\right) -1\right],
	\label{ScalingFunction}
\end{equation}
where $C$ is a phenomenological parameter and $b$ is a shift exponent~\cite{Fisher:1972zza}. This modification comes from the fact that the position of the maximum of $\chi_m$ is volume dependent. Due to this modification, the critical temperature can be extracted directly in infinite volume. The O(4) model does not show any shift of the maximum and hence Eq.~(\ref{eq:susc_scaling}) is valid here. It should be noted, that the temperature plays either the role of $y$ in the Higgs-Yukawa model or $\kappa$ in the O(4) model.
%\newpage %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To extract the critical exponents from susceptibility, we perform a simultaneous fit to all volumes to the partly-empirical formula~\cite{Jansen:1989gd},
\begin{align}
	\chi_{m} = A\left(L_s^{-2/\nu} + B\left[T/T_c^{(L=\infty)} - C\cdot L_{s}^{-b}-1\right]^2\right)^{-\gamma/2}.
	\label{FitFunction}
\end{align}
This formula was also used for a fit to $\chi_m$ of the O(4) model, but with the modification of excluding the parameters $C$ and $b$ because of the reasons mentioned above. The fit results are summarized in TABLE~\ref{TableFitSus} and will be discussed later.

%%%%%%%%%%%%%%%%%%%%%%
%Picture%%%%% Susceptibility at large Y
\begin{figure}[H]
	\begin{center}
	$	
	\begin{array}{ccc}
		\hspace*{-0.5cm} \input{pictures/StrongYukawaCoupling/susceptibility_kap006.tex} &
		\hspace*{-1.2cm} \input{pictures/StrongYukawaCoupling/susceptibility_kap000.tex} &
		\hspace*{-1.2cm} \input{pictures/StrongYukawaCoupling/susceptibility_O4.tex} 
	\end{array}
	$	
	\end{center}
\vspace*{-0.5cm}
\caption[Susceptibility at large Yukawa couplings.]{Susceptibility $\chi_m$ at $\kappa=0.06$ (left), $\kappa=0.00$ (middle) and the O(4) model (right) for various volumes. The curves are the result of a fit to Eq.~(\ref{FitFunction}). The right top boxes in the middle and the right picture show $\chi_m$ for the largest volumes. For the Higgs-Yukawa model a volume dependent shift of $y_c$ towards $y_c^{(L=\infty)}$ can be observed which is absent in the O(4) model.}	
\label{SusAtLargeY}
\end{figure} %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%
%Table%%%%%%%% fit results %%%%%%%%%
\begin{table}[H]\centering{
	\begin{tabular}{|c||c|c|c|c|c|c||c|}\hline
		& $T_c^{(L=\infty)}$ & $\nu$ & $\gamma$ & $C$ & $b$ & $\chi^2/\text{d.o.f.}$ & fit interval \\ \hline\hline
		$\kappa=0.06$ & 18.119(67) & 0.576(28) & 1.038(30) & 4.7(1.6) & 1.95(18) & 0.184 & 17.5, 20.0 \\ \hline   
		$\kappa=0.00$ & 16.676(15) & 0.541(22) & 0.996(15) & 10(2) & 2.42(1) & 0.160 & 15.0, 19.0\\ \hline  
		O(4)                    & 0.304268(27) & 0.499(12) & 1.086(19) & X & X & 0.204 & 0.300, 0.308 \\ \hline
	\end{tabular}}
\caption[Fit results to Eq.~(\ref{FitFunction}).]{Results of a correlated fit to the susceptibility according to Eq.~(\ref{FitFunction}) where the last row indicates the fit interval. The parameter $T$ stands either for $y$ in the Higgs-Yukawa model or for $\kappa$ in the O(4) model. Since no volume dependent shift can be observed in the O(4) model for $\chi_m$, the parameters $C$ and $b$ have not been fitted here. All quoted errors are statistically only.}	
\label{TableFitSus}
\end{table}%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

It is possible to rescale the susceptibility according to Eq.~(\ref{ScalingFunction}), or Eq.~(\ref{eq:susc_scaling}) for the O(4) model respectively. The fitted parameters extracted from Eq.~(\ref{FitFunction}) can be used to construct $\chi_{m}\left(t, L\right)\cdot L_s^{-\gamma/\nu}$ and test its scaling against $t\cdot L_s^{1/\nu}$. This scaling test is shown in FIG.~\ref{SusRescaledAtLargeY}. Points for all volumes collapse on the same curve in the three cases shown. This behavior is typical for second order phase transitions and hence another strong evidence that such a transition happens.

%%%%%%%%%%%%%%%%%%%%%%
%Picture%%%%% Susceptibility: Rescaled
\begin{figure}[H]
	\begin{center}
	$	
	\begin{array}{ccc}
		\hspace*{-0.5cm}  \input{pictures/StrongYukawaCoupling/sus_rescaled_kap006.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/sus_rescaled_kap000.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/sus_rescaled_O4.tex} 
	\end{array}
	$	
	\end{center}
\vspace*{-0.5cm}
\caption[Rescaled susceptibility at large Yukawa couplings.]{Scaling behavior of susceptibility at $\kappa=0.06$ (left), $\kappa=0.00$ (middle) and the O(4) model (right) for various volumes.}
\label{SusRescaledAtLargeY}
\end{figure} %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

An alternative way of determining critical exponents is via Binder's cumulant, Eq.~(\ref{eq:binders_cumulant_def}). 
The great advantage of this quantity is the scaling invariance close to the critical point,
\begin{equation}
\label{eq:Binder_cumulant_scaling}
	Q_L  = g_{Q_L}\left( tL^{1/\nu}\right),
\end{equation}
where $g_{Q_L}$ is the scaling function of Binder's cumulant. This behavior can be observed in FIG. \ref{BinderAtLargeY} where all volumes intersect at the phase transition point in infinite volume (see the boxes in the upper right corner). Even for the Higgs-Yukawa model no shift can be observed and hence the parameters $C$ and $b$ can be neglected.

The value of Binder's cumulant in the broken phase comes from the fact that $\left< m^4\right>\approx\left< m^2\right>^2$ and hence $Q_L\approx2/3$ \cite{Binder:1981sa}. However, the values of $Q_L$ at the critical point in the Higgs-Yukawa model differ from the one in the O(4) model. This might be due to finite renormalization of fermions or, since $Q_L$ is proportional to the renormalized quartic coupling, this might give an additional hint on the difference between the O(4) model and the region of large unrenormalized Yukawa couplings. However, this must be postponed to later studies. 

%%%%%%%%%%%%%%%%%%%%%%%%
%Picture%%%%% Binder Cumulant at large Y 
\begin{figure}[H]
	\begin{center}
	$	
	\begin{array}{ccc}
		\hspace*{-0.5cm}  \input{pictures/StrongYukawaCoupling/binder_kap006.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/binder_kap000.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/binder_O4.tex} 
	\end{array}
	$	
	\end{center}
\vspace*{-0.5cm}
\caption[Binder cumulant at large Yukawa couplings.]{Binder's Cumulant $Q_L$ at $\kappa=0.06$ (left), $\kappa=0.00$ (middle) and the O(4) model (right) for various volumes where the subscript L indicates the finite volume quantity. The values of $Q_L$ in the Higgs-Yukawa and the O(4) models differ at the critical point.}	
\label{BinderAtLargeY}
\end{figure} %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%

The basic idea of extracting the critical exponent, $\nu$, from Binder's cumulant is the use of the curve collapse of Eq.~(\ref{ScalingFunction}). If the scaling function $g_{Q_L}$ is known one could simply minimize \cite{0305-4470-34-33-302}
\begin{equation}
	R_{Q_L} =\frac{1}{N}\sum\left| Q_L - g_{Q_L}\left(tL^{1/\nu}\right)\right|,
	\label{BinderMinimizationWithKnowng}
\end{equation}
what is a direct consequence of the scaling behavior. The sum is taken over all data points $N$ and it is minimal for the correct choice of the parameters $\nu$ and $T_c^{L=\infty}$. In absence of any statistical and systematic errors the function $R_{Q_L}$ would become zero. 

The scaling function $g_{Q_L}$ is unknown. However, this can be overcome by the observation that any volume, in the following called $p$, can act as this function for the correct choice of parameters. Instead of minimizing Eq.~(\ref{BinderMinimizationWithKnowng}), we minimize
\begin{equation}
	P_b = \left[ \frac{1}{N_\text{over}}\sum_p\sum_{j\ne p}\sum_{i, \text{over}} \left| Q_{L_j}- \mathcal{E}_p\left( t_{ij} L_j^{1/\nu} \right) \right|^2 \right]^{1/2}.
\end{equation}
Here, the scaling function is replaced by the interpolating function $\mathcal{E}_p$ which is based on the values of volume $p$ but evaluated at points $t_{ij} L_j^{1/\nu}$ of volume $j$. In our case, $\mathcal{E}_p$ is computed by picking a point in $j$ and taking the four neighboring points in $p$ as a basis for a quadratic interpolation. The index $i$ counts all points in volume $j$ and the normalization factor $N_\text{over}$ is the total number points used to evaluate $\mathcal{E}_p$. The results are summarized in TABLE~\ref{TablePBmini} and the curve collapse for Binder's cumulant is shown in FIG.~\ref{BinderRescaledAtLargeY}.

In principle, this method could also be used for $\chi_m$ but instead of minimizing $P_B$ for only two parameters it would be necessary to minimize for five parameters. It turned out that this leads to numerical instabilities and the extraction of critical exponents from the susceptibility is not possible so far. \\
%%%%%%%%%%%%%%%%%%%%%%%%%%
%Table%%%%%%%% fit results %%%%%%%%%
\begin{table}[H]
	\centering{
	\begin{tabular}{|c||c|c||c|}\hline
		& $T_c^{(L=\infty)}$ & $\nu$ & interval \\ \hline\hline
		$\kappa=0.06$ & 18.147(24) & 0.550(1) & 17.4, 18.8 \\ \hline   
		$\kappa=0.00$ & 16.667(27) & 0.525(6) & 16.0, 17.2 \\ \hline  
		O(4)                    & 0.3005(34) & 0.50000(3) & 0.294, 0.314 \\ \hline 
	\end{tabular}}
\caption[Curve collapse results of Binder cumulant.]{Curve collapse results of Binder's cumulant where the last row indicates the interval in which the procedure has been used. The parameter $T$ stands either for $y$ in the Higgs-Yukawa model or for $\kappa$ in the O(4) model. All errors are statistically only.}
\label{TablePBmini}
\end{table}%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%Picture%%%%% Binder Cumulant rescaled 
\begin{figure}[H]
	\begin{center}
	$	
	\begin{array}{ccc}
		\hspace*{-0.5cm}  \input{pictures/StrongYukawaCoupling/binder_rescaled_kap006.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/binder_rescaled_kap000.tex} &
		\hspace*{-1.2cm}  \input{pictures/StrongYukawaCoupling/binder_rescaled_O4.tex} 
	\end{array}
	$	
	\end{center}
\vspace*{-0.5cm}
\caption[Scaling behaviour of Binder cumulant at large Yukawa couplings.]{Scaling behavior of Binder's cumulant at $\kappa=0.06$ (left), $\kappa=0.00$ (middle) and the O(4) model (right) for various volumes.}	
\label{BinderRescaledAtLargeY}
\end{figure} %%%%%%%%%%%%%%%%

At this point we can claim, that we found a second order phase transition in the strong Yukawa coupling regime. The absence of discontinuities in $\left<m\right>$ and the perfect finite size scaling of $\chi_m$ are evidence strong enough for such a statement. So it is valid to compare the critical exponents extracted from susceptibility and Binder's cumulant with the ones of the standard model and hence the O(4) model. 

To be able to make a direct comparison of the O(4) model with the Higgs-Yukawa model, the same program has been used to compute observables. Furthermore, the same analysis techniques have been used. The results of the correlated fit to $\chi_m$ are summarized in TABLE~\ref{TableFitSus}. The errors quoted there are purely statistical. Investigation of the dependence of the fit on the fit interval leads to systematic uncertainties which are as large as the statistical errors roughly. It is not possible to claim a significant difference in the critical exponents from this method so far.

The curve collapse method, however, can only provide us with information about one critical exponent, namely $\nu$. The advantage of this method is the much smaller statistical error compared to the fit to $\chi_m$ but it must be used with some care. The scaling behavior claimed in Eq.~(\ref{eq:Binder_cumulant_scaling}) is only true close to the critical point. If this method is applied at points too far away form the phase transition the result can be spoiled by finite size effects. One possibility to get an impression of the dependence of the interval in which the curve collapse method works is to vary the interval. It was found, that the systematic uncertainty is roughly a factor of five larger than the statistical. However, in the case of $\kappa=0.06$ and of the O(4) model the total error is a factor of five smaller compared to the fitting procedure. In the case of $\kappa=0.00$ the total errors are compatible. 

We cannot claim a clear difference of the Higgs-Yukawa model at large unrenormalized Yulawa couplings from the O(4) model at this point, although we see evidence of it. The critical exponents in the strong coupling region and the O(4) model are different but the deviation is not strong enough within the statistical and systematic errors. We will increase statistics in the future and will improve on the methods to extract the critical exponents. This will allow us to give a final statement if the sector of large unrenormalized Yukawa couplings is indeed different from the standard model sector.



















==> figures/binder_kap000.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$Q_L$}}}%
      \put(2185,305){\makebox(0,0){\strut{}$y$}}%
      \put(972,1949){\makebox(0,0)[l]{\strut{}\textcolor{gray}{\boldmath{$\kappa=0.00$}}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1387,1190){\makebox(0,0)[r]{\strut{}L=8}}%
      \csname LTb\endcsname%
      \put(1387,1036){\makebox(0,0)[r]{\strut{}L=12}}%
      \csname LTb\endcsname%
      \put(1387,882){\makebox(0,0)[r]{\strut{}L=16}}%
      \csname LTb\endcsname%
      \put(1387,728){\makebox(0,0)[r]{\strut{}L=24}}%
      \csname LTb\endcsname%
      \put(831,580){\makebox(0,0)[r]{\strut{}0.48}}%
      \csname LTb\endcsname%
      \put(831,978){\makebox(0,0)[r]{\strut{}0.52}}%
      \csname LTb\endcsname%
      \put(831,1376){\makebox(0,0)[r]{\strut{}0.56}}%
      \csname LTb\endcsname%
      \put(831,1775){\makebox(0,0)[r]{\strut{}0.60}}%
      \csname LTb\endcsname%
      \put(831,2173){\makebox(0,0)[r]{\strut{}0.64}}%
      \csname LTb\endcsname%
      \put(831,2571){\makebox(0,0)[r]{\strut{}0.68}}%
      \csname LTb\endcsname%
      \put(858,470){\makebox(0,0){\strut{} 14}}%
      \csname LTb\endcsname%
      \put(1237,470){\makebox(0,0){\strut{} 15}}%
      \csname LTb\endcsname%
      \put(1617,470){\makebox(0,0){\strut{} 16}}%
      \csname LTb\endcsname%
      \put(1996,470){\makebox(0,0){\strut{} 17}}%
      \csname LTb\endcsname%
      \put(2375,470){\makebox(0,0){\strut{} 18}}%
      \csname LTb\endcsname%
      \put(2754,470){\makebox(0,0){\strut{} 19}}%
      \csname LTb\endcsname%
      \put(3134,470){\makebox(0,0){\strut{} 20}}%
      \csname LTb\endcsname%
      \put(3513,470){\makebox(0,0){\strut{} 21}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \tiny
      \put(2527,2030){\makebox(0,0)[r]{\strut{}0.658}}%
      \put(2527,2389){\makebox(0,0)[r]{\strut{}0.664}}%
      \put(2707,1762){\makebox(0,0){\strut{} 16.2}}%
      \put(3030,1762){\makebox(0,0){\strut{} 16.5}}%
      \put(3353,1762){\makebox(0,0){\strut{} 16.8}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{binder_kap000}}%
    \gplfronttext
  \end{picture}%
\endgroup



==> figures/binder_kap006.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$Q_L$}}}%
      \put(2185,305){\makebox(0,0){\strut{}$y$}}%
      \put(981,1949){\makebox(0,0)[l]{\strut{}\textcolor{gray}{\boldmath{$\kappa=0.06$}}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1379,1036){\makebox(0,0)[r]{\strut{}L=8}}%
      \csname LTb\endcsname%
      \put(1379,882){\makebox(0,0)[r]{\strut{}L=12}}%
      \csname LTb\endcsname%
      \put(1379,728){\makebox(0,0)[r]{\strut{}L=16}}%
      \csname LTb\endcsname%
      \put(831,580){\makebox(0,0)[r]{\strut{}0.48}}%
      \csname LTb\endcsname%
      \put(831,978){\makebox(0,0)[r]{\strut{}0.52}}%
      \csname LTb\endcsname%
      \put(831,1376){\makebox(0,0)[r]{\strut{}0.56}}%
      \csname LTb\endcsname%
      \put(831,1775){\makebox(0,0)[r]{\strut{}0.60}}%
      \csname LTb\endcsname%
      \put(831,2173){\makebox(0,0)[r]{\strut{}0.64}}%
      \csname LTb\endcsname%
      \put(831,2571){\makebox(0,0)[r]{\strut{}0.68}}%
      \csname LTb\endcsname%
      \put(858,470){\makebox(0,0){\strut{} 16}}%
      \csname LTb\endcsname%
      \put(1266,470){\makebox(0,0){\strut{} 17}}%
      \csname LTb\endcsname%
      \put(1675,470){\makebox(0,0){\strut{} 18}}%
      \csname LTb\endcsname%
      \put(2083,470){\makebox(0,0){\strut{} 19}}%
      \csname LTb\endcsname%
      \put(2492,470){\makebox(0,0){\strut{} 20}}%
      \csname LTb\endcsname%
      \put(2900,470){\makebox(0,0){\strut{} 21}}%
      \csname LTb\endcsname%
      \put(3309,470){\makebox(0,0){\strut{} 22}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \tiny
      \put(2527,2030){\makebox(0,0)[r]{\strut{}0.658}}%
      \put(2527,2389){\makebox(0,0)[r]{\strut{}0.664}}%
      \put(2597,1762){\makebox(0,0){\strut{} 17.7}}%
      \put(2981,1762){\makebox(0,0){\strut{} 18.1}}%
      \put(3365,1762){\makebox(0,0){\strut{} 18.5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{binder_kap006}}%
    \gplfronttext
  \end{picture}%
\endgroup



==> figures/finiteT_2/finiteT_mt175_T4_scale.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$\Lambda \text{ in GeV}$}}}%
      \put(2251,354){\makebox(0,0){\strut{}$L^{2}$}}%
      \put(2554,2191){\makebox(0,0)[l]{\strut{}\textcolor{gray}{\bf $L_t=4$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2178,1077){\makebox(0,0)[r]{\strut{}$\kappa=0.3013$}}%
      \csname LTb\endcsname%
      \put(2178,923){\makebox(0,0)[r]{\strut{}$\kappa=0.3014$}}%
      \csname LTb\endcsname%
      \put(2178,769){\makebox(0,0)[r]{\strut{}$\kappa=0.3015$}}%
      \csname LTb\endcsname%
      \put(963,629){\makebox(0,0)[r]{\strut{} 1700}}%
      \csname LTb\endcsname%
      \put(963,1102){\makebox(0,0)[r]{\strut{} 1800}}%
      \csname LTb\endcsname%
      \put(963,1576){\makebox(0,0)[r]{\strut{} 1900}}%
      \csname LTb\endcsname%
      \put(963,2049){\makebox(0,0)[r]{\strut{} 2000}}%
      \csname LTb\endcsname%
      \put(963,2522){\makebox(0,0)[r]{\strut{} 2100}}%
      \csname LTb\endcsname%
      \put(990,519){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1495,519){\makebox(0,0){\strut{} 0.001}}%
      \csname LTb\endcsname%
      \put(1999,519){\makebox(0,0){\strut{} 0.002}}%
      \csname LTb\endcsname%
      \put(2504,519){\makebox(0,0){\strut{} 0.003}}%
      \csname LTb\endcsname%
      \put(3008,519){\makebox(0,0){\strut{} 0.004}}%
      \csname LTb\endcsname%
      \put(3513,519){\makebox(0,0){\strut{} 0.005}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{finiteT_mt175_T4_scale}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/finiteT_2/finiteT_mt175_infKappa.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$\kappa_c$}}}%
      \put(2251,354){\makebox(0,0){\strut{}$L^{-1/\nu}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1650,923){\makebox(0,0)[r]{\strut{}$L_t=4$}}%
      \csname LTb\endcsname%
      \put(1650,769){\makebox(0,0)[r]{\strut{}$L_t=6$}}%
      \csname LTb\endcsname%
      \put(963,629){\makebox(0,0)[r]{\strut{}0.298}}%
      \csname LTb\endcsname%
      \put(963,1102){\makebox(0,0)[r]{\strut{}0.299}}%
      \csname LTb\endcsname%
      \put(963,1576){\makebox(0,0)[r]{\strut{}0.300}}%
      \csname LTb\endcsname%
      \put(963,2049){\makebox(0,0)[r]{\strut{}0.301}}%
      \csname LTb\endcsname%
      \put(963,2522){\makebox(0,0)[r]{\strut{}0.302}}%
      \csname LTb\endcsname%
      \put(990,519){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1621,519){\makebox(0,0){\strut{} 0.005}}%
      \csname LTb\endcsname%
      \put(2252,519){\makebox(0,0){\strut{} 0.01}}%
      \csname LTb\endcsname%
      \put(2882,519){\makebox(0,0){\strut{} 0.015}}%
      \csname LTb\endcsname%
      \put(3513,519){\makebox(0,0){\strut{} 0.02}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{finiteT_mt175_infKappa}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/finiteT_2/finiteT_mt675_T4_susc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$\chi_m$}}}%
      \put(2119,255){\makebox(0,0){\strut{}$\kappa$}}%
      \put(2567,1656){\makebox(0,0)[l]{\strut{}\textcolor{gray}{\bf $L_t=4$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2905,2481){\makebox(0,0)[r]{\strut{}L=16}}%
      \csname LTb\endcsname%
      \put(2905,2327){\makebox(0,0)[r]{\strut{}L=20}}%
      \csname LTb\endcsname%
      \put(2905,2173){\makebox(0,0)[r]{\strut{}L=24}}%
      \csname LTb\endcsname%
      \put(699,530){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(699,852){\makebox(0,0)[r]{\strut{} 2}}%
      \csname LTb\endcsname%
      \put(699,1173){\makebox(0,0)[r]{\strut{} 4}}%
      \csname LTb\endcsname%
      \put(699,1495){\makebox(0,0)[r]{\strut{} 6}}%
      \csname LTb\endcsname%
      \put(699,1817){\makebox(0,0)[r]{\strut{} 8}}%
      \csname LTb\endcsname%
      \put(699,2138){\makebox(0,0)[r]{\strut{} 10}}%
      \csname LTb\endcsname%
      \put(699,2460){\makebox(0,0)[r]{\strut{} 12}}%
      \csname LTb\endcsname%
      \put(925,420){\makebox(0,0){\strut{}0.16}}%
      \csname LTb\endcsname%
      \put(1323,420){\makebox(0,0){\strut{}0.18}}%
      \csname LTb\endcsname%
      \put(1721,420){\makebox(0,0){\strut{}0.20}}%
      \csname LTb\endcsname%
      \put(2120,420){\makebox(0,0){\strut{}0.22}}%
      \csname LTb\endcsname%
      \put(2518,420){\makebox(0,0){\strut{}0.24}}%
      \csname LTb\endcsname%
      \put(2916,420){\makebox(0,0){\strut{}0.26}}%
      \csname LTb\endcsname%
      \put(3314,420){\makebox(0,0){\strut{}0.28}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{finiteT_mt675_T4_susc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/finiteT_2/finiteT_mt675_T6_susc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$\chi_m$}}}%
      \put(2119,255){\makebox(0,0){\strut{}$\kappa$}}%
      \put(2567,1656){\makebox(0,0)[l]{\strut{}\textcolor{gray}{\bf $L_t=6$}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2905,2481){\makebox(0,0)[r]{\strut{}L=16}}%
      \csname LTb\endcsname%
      \put(2905,2327){\makebox(0,0)[r]{\strut{}L=20}}%
      \csname LTb\endcsname%
      \put(2905,2173){\makebox(0,0)[r]{\strut{}L=24}}%
      \csname LTb\endcsname%
      \put(699,530){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(699,852){\makebox(0,0)[r]{\strut{} 2}}%
      \csname LTb\endcsname%
      \put(699,1173){\makebox(0,0)[r]{\strut{} 4}}%
      \csname LTb\endcsname%
      \put(699,1495){\makebox(0,0)[r]{\strut{} 6}}%
      \csname LTb\endcsname%
      \put(699,1817){\makebox(0,0)[r]{\strut{} 8}}%
      \csname LTb\endcsname%
      \put(699,2138){\makebox(0,0)[r]{\strut{} 10}}%
      \csname LTb\endcsname%
      \put(699,2460){\makebox(0,0)[r]{\strut{} 12}}%
      \csname LTb\endcsname%
      \put(925,420){\makebox(0,0){\strut{}0.16}}%
      \csname LTb\endcsname%
      \put(1323,420){\makebox(0,0){\strut{}0.18}}%
      \csname LTb\endcsname%
      \put(1721,420){\makebox(0,0){\strut{}0.20}}%
      \csname LTb\endcsname%
      \put(2120,420){\makebox(0,0){\strut{}0.22}}%
      \csname LTb\endcsname%
      \put(2518,420){\makebox(0,0){\strut{}0.24}}%
      \csname LTb\endcsname%
      \put(2916,420){\makebox(0,0){\strut{}0.26}}%
      \csname LTb\endcsname%
      \put(3314,420){\makebox(0,0){\strut{}0.28}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{finiteT_mt675_T6_susc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/finiteT_2/finiteT_mt675_infKappa.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3910.00,2976.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(352,1575){\rotatebox{-270}{\makebox(0,0){\strut{}$\kappa_c$}}}%
      \put(2251,354){\makebox(0,0){\strut{}$L^{-1/\nu}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1650,2382){\makebox(0,0)[r]{\strut{}$L_t=4$}}%
      \csname LTb\endcsname%
      \put(1650,2228){\makebox(0,0)[r]{\strut{}$L_t=6$}}%
      \csname LTb\endcsname%
      \put(963,629){\makebox(0,0)[r]{\strut{}0.211}}%
      \csname LTb\endcsname%
      \put(963,945){\makebox(0,0)[r]{\strut{}0.212}}%
      \csname LTb\endcsname%
      \put(963,1260){\makebox(0,0)[r]{\strut{}0.213}}%
      \csname LTb\endcsname%
      \put(963,1576){\makebox(0,0)[r]{\strut{}0.214}}%
      \csname LTb\endcsname%
      \put(963,1891){\makebox(0,0)[r]{\strut{}0.215}}%
      \csname LTb\endcsname%
      \put(963,2207){\makebox(0,0)[r]{\strut{}0.216}}%
      \csname LTb\endcsname%
      \put(963,2522){\makebox(0,0)[r]{\strut{}0.217}}%
      \csname LTb\endcsname%
      \put(990,519){\makebox(0,0){\strut{} 0}}%
      \csname LTb\endcsname%
      \put(1621,519){\makebox(0,0){\strut{} 0.005}}%
      \csname LTb\endcsname%
      \put(2252,519){\makebox(0,0){\strut{} 0.01}}%
      \csname LTb\endcsname%
      \put(2882,519){\makebox(0,0){\strut{} 0.015}}%
      \csname LTb\endcsname%
      \put(3513,519){\makebox(0,0){\strut{} 0.02}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{finiteT_mt675_infKappa}}%
    \gplfronttext
  \end{picture}%
\endgroup

